Optimizing the Expected Mean Payoff in Energy Markov Decision Processes

Energy Markov Decision Processes (EMDPs) are finite-state Markov decision processes where each transition is assigned an integer counter update and a rational payoff. An EMDP configuration is a pair s(n), where s is a control state and n is the current counter value. The configurations are changed by performing transitions in the standard way. We consider the problem of computing a safe strategy (i.e., a strategy that keeps the counter non-negative) which maximizes the expected mean payoff.

==> pump-compute.tex <==
We reduce the problem of computing $\minpump$ to the problem of computing minimal initial credit in \emph{energy parity MDPs}~\cite{CHD:energy-MDPs}, where we are required to find a safe strategy which visits with probability 1 a given set of states infinitely often. Given an EMDP $\calE$ we construct a new EMDP $\calE$ by adding new states and transitions to $\calE$. For each transition $e=(s,t)$ of $\calE$ we add new controllable states $s_e,s'_e$ and transitions $(s,s_e),(s_e,t)$, $(s_e,s'_e)$, $(s'_e,s_e)$ such that $E(s_e,s'_e)=-1$ and the other three transitions have energy update 0 (the reward of the new transitions is irrelevant). We require that some state if the form $s'_e$ is visited infinitely often, i.e. that the counter is infinitely often decreased by 1. It is easy to verify that a configuration is pumpable if and only if it admits a safe strategy that satisfies this B\"uchi objective with probability one. 

To determine minimal initial energy level needed to achieve the latter, in~\cite{CHD:energy-MDPs} they provide a polynomial reduction to determining the minimal initial level in energy B\"uchi games, a problem which is shown to be solvable by an $\PTIME^{\EG}$ algorithm in \cite{CD:energy-parity-games}. Now from the results of~\cite{CD:energy-parity-games} it follows that there is a memoryless \emph{good-for-energy} strategy $\iota$ having the following property in every pumpable configuration: each cycle traversed under $\iota$ either strictly increases the counter, or has zero net effect on the counter but visits an B\"uchi-accepting state. But in $\calE'$ no such strategy can reach any B\"uchi state $s'_e$, as this would close a negative cycle $s'_e,s_e,s'_e$ (due to memorylessness). Hence, $\iota$ ensures that each reachable cycle has positive effect on the counter, hence, it is a memoryless globally pumping strategy.

